A posteriori error estimates for finite element exterior calculus: The de Rham complex

Finite element exterior calculus (FEEC) has been developed over the past decade as a framework for constructing and analyzing stable and accurate numerical methods for partial differential equations by employing differential complexes. The recent work of Arnold, Falk and Winther \cite{ArFaWi2010} includes a well-developed theory of finite element methods for Hodge Laplace problems, including a priori error estimates. In this work we focus on developing a posteriori error estimates in which the computational error is bounded by some computable functional of the discrete solution and problem data. More precisely, we prove a posteriori error estimates of residual type for Arnold-Falk-Winther mixed finite element methods for Hodge-de Rham Laplace problems. While a number of previous works consider a posteriori error estimation for Maxwell's equations and mixed formulations of the scalar Laplacian, the approach we take is distinguished by unified treatment of the various Hodge Laplace problems arising in the de Rham complex, consistent use of the language and analytical framework of differential forms, and the development of a posteriori error estimates for harmonic forms and the effects of their approximation on the resulting numerical method for the Hodge Laplacian.

==> alandefs.tex <==
\def\dx{\hspace{2pt}{\rm d}x}
\def\d{\hspace{2pt}{\rm d}}
\def\vp{\vec{p}}
\def\vr{\vec{r}}
\def\tr{\tilde{r}}
\def\vq{\vec{q}}
\def\vQ{\vec{Q}}
\def\vz{\vec{z}}
\def\dels{\delta^0}
\def\delv{\vec{\delta}^0_i}
\def\tp{\tilde{p}}
\def\vb{\vec{b}}
\def\hc{\hat{c}}
\def\l2{_{L_2(\Omega)}}
\def\nl2{_{[L_2(\Omega)]^n}}
\setlength{\arraycolsep}{.5mm}
\def\td{\tilde{\delta}^{x_0}}
\def\tg{\tilde{g}}
\def\hmin{\underline{h}}
\def\hmax{\overline{h}}
\def\E{\mathcal{E}}
\def\ellh{\ell_{\hmin,n}}
\setlength{\arraycolsep}{.3mm}
\setlength{\extrarowheight}{.5mm}

\def\Xint#1{\mathchoice {\XXint\displaystyle\textstyle{#1}}% 
{\XXint\textstyle\scriptstyle{#1}}% 
{\XXint\scriptstyle\scriptscriptstyle{#1}}% 
{\XXint\scriptscriptstyle\scriptscriptstyle{#1}}% 
\!\int} \def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$} 
\vcenter{\hbox{$#2#3$}}\kern-.5\wd0}} 
\def\ddashint{\Xint=} 
\def\dashint{\Xint-} 

\newcommand{\mat}[2][rrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr]{\left [
	 \begin{array}{#1}
	 #2\\ 
	 \end{array}
	 \right ] }


\def\T{\mathcal{T}}
\def\N{\mathcal{N}}
\def\dv{\rm{div}}
%\def\det{\rm{det}}

\def\B{\mathfrak{B}}
\def\H{\mathfrak{H}}
\def\Z{\mathfrak{Z}}


==> defs.tex <==
% General math commands
\DeclareMathOperator{\sgn}{sgn}
\def\st{\, |\,}

% Spaces
\def\R{\mathbb{R}}
\def\Real{\mathbb{R}}
\def\RR{\mathbb{R}}
\def\Z{\mathbb{Z}}
\def\F{\mathbb{F}}
\def\Q{\mathbb{Q}}

% Function spaces
\newcommand{\Lforms}[2]{L^#1\Omega^#2\bigl(\abs{K}\bigr)}

% Functions
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\supp}{supp} % already defined in defs.tex

% Linear algebra
\DeclareMathOperator{\diag}{diag} % already defined in defs.tex
\DeclareMathOperator{\rank}{rank}

% Point-set topology
\DeclareMathOperator{\cl}{cl}

% Homological algebra
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Ext}{Ext}


% Vector calculus
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\boldcurl}{\bf curl}
\def\div{\operatorname{div}}
\DeclareMathOperator{\D}{D}

% Simplices and simplicial complexes
\newcommand{\vol}[1]{\abs{#1}}
\newcommand{\simplex}[1]{[v_0,\ldots,v_{#1}]}
\newcommand{\Simplex}[1]{\bigl[v_0,\ldots,v_{#1}\bigr]}
\newcommand{\hasface}{\succeq}
\newcommand{\faceof}{\preceq}
\newcommand{\hasprprface}{\succ}
\newcommand{\prprfaceof}{\prec}
\DeclareMathOperator{\Bd}{Bd}
\DeclareMathOperator{\Int}{Int}
\DeclareMathOperator{\St}{St}
\DeclareMathOperator{\ClSt}{\overline{St}}
\DeclareMathOperator{\Lk}{Lk}
\DeclareMathOperator{\affine}{aff}
\newcommand{\cone}[2]{\ensuremath{#1 * #2}}
\newcommand{\eqB}{\ensuremath{B}}
\newcommand{\meshM}{\ensuremath{\mathcal{M}}}


% Exterior calculus 
\def\d{\operatorname{d}}
\def\ud{\ensuremath{\mathrm{d}}}
\DeclareMathOperator{\codiff}{\delta} 
\DeclareMathOperator{\dcodiff}{\delta}
\DeclareMathOperator{\dd}{d} 
\DeclareMathOperator{\hodge}{\ast} 
\DeclareMathOperator{\dual}{\star}
\DeclareMathOperator{\laplacian}{\Delta}
\DeclareMathOperator{\deRham}{R}
\DeclareMathOperator{\whitney}{W}

% Algebraic topology 
\DeclareMathOperator{\boundary}{\partial}
\DeclareMathOperator{\coboundary}{\delta}
\newcommand{\cochainBasis}[2]{\bigl(\sigma^#1_#2\bigr)^\ast}
\newcommand{\rltvbndry}[3]{\operatorname{\boundary}_{#1}^{\, (#2,#3)}}

% Finite elements
\def\P{\mathcal{P}}
\def\T{\mathcal{T}}

% Delimiters
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\matrixform}[1]{\left[ #1 \right]}

% Inner products
\newcommand{\eval}[2]{\langle #1,#2 \rangle}
\newcommand{\Eval}[2]{\bigl\langle #1,#2 \bigr\rangle}
\newcommand{\innerproduct}[2]{\langle #1, #2 \rangle}
\newcommand{\Innerproduct}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\ainnerproduct}[2]{\langle #1, #2 \rangle}
\newcommand{\aInnerproduct}[2]{\bigl\langle #1, #2 \bigr\rangle}
\newcommand{\pinnerproduct}[2]{( #1, #2 )}
\newcommand{\pInnerproduct}[2]{\bigl( #1, #2 \bigr)}

% Formatting commands
\def\p{\phantom{-}}

% Paper editing commands
\newcommand{\todo}[1]{\vspace{5 mm}\par \noindent
\marginpar{\textsc{ToDo}}
\framebox{\begin{minipage}[c]{0.95 \textwidth}
\tt #1 \end{minipage}}\vspace{5 mm}\par}
\newcommand{\achtung}[2]{\vspace{5 mm}\par \noindent
\marginpar{\textsc{#1}}
\framebox{\begin{minipage}[c]{0.95 \textwidth}
\textsf{#2} \end{minipage}}\vspace{5 mm}\par}
\newcommand{\marginnote}[1]{\marginpar{\scriptsize\textsf{#1}}}

% Bold alphabet for use in mathematics
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cc}{\mathbf{c}}
\newcommand{\ee}{\mathbf{e}}
\newcommand{\ff}{\mathbf{f}}
\newcommand{\uu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\ww}{\mathbf{w}}
\newcommand{\xx}{\mathbf{x}}
\newcommand{\yy}{\mathbf{y}}
\newcommand{\zz}{\mathbf{z}}

% Footnote with symbol
\long\def\symbolfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}

% % Nathan Dunfield's basic label overlay environment.  The usual
% % version is the second one below.  Args are: coor system, graphics
% % modifiers, graphics name

% \usepackage[import]{xy}
% \newenvironment{xyoverpic}[3]
% {%
% \begin{xy}
% \xyimport#1{\includegraphics[#2]{#3}}
% }{\end{xy}}

% \newenvironment{cxyoverpic}[3]
% {%
% \begin{center}
% \centering\leavevmode\small
% \begin{xyoverpic}{#1}{#2}{#3}
% }{\end{xyoverpic}
% \end{center}}

% Editing commands requiring color package -- copy into document and uncomment
% \newcommand{\add}[1]{\textcolor{blue}{#1}}
% \newcommand{\delete}[1]{\textcolor{red}{#1}}
% \definecolor{darkgrn}{rgb}{0, 0.75, 0}
% \newcommand{\modified}[1]{\textcolor{darkgrn}{#1}}

% Editing instructions for co-authors, copy into document and uncomment
% \achtung{ANH}{
%   \noindent  \modified{This color means MODIFIED, use
%   \textbackslash modified\{text\}}\\
%   \noindent \delete{This color means DELETE, use 
%     \textbackslash delete\{text\}}\\
%   \noindent \add{This color means ADD, use \textbackslash
%     add\{text\}}
% }



